Do Text Simplification Systems Preserve Meaning? A Human Evaluation via Reading Comprehension

Automatic text simplification (TS) aims to automate the process of rewriting text to make it easier for people to read. A pre-requisite for TS to be useful is that it should convey information that is consistent with the meaning of the original text. However, current TS evaluation protocols assess system outputs for simplicity and meaning preservation without regard for the document context in which output sentences occur and for how people understand them. In this work, we introduce a human evaluation framework to assess whether simplified texts preserve meaning using reading comprehension questions. With this framework, we conduct a thorough human evaluation of texts by humans and by nine automatic systems. Supervised systems that leverage pre-training knowledge achieve the highest scores on the reading comprehension (RC) tasks amongst the automatic controllable TS systems. However, even the best-performing supervised system struggles with at least 14% of the questions, marking them as "unanswerable'' based on simplified content. We further investigate how existing TS evaluation metrics and automatic question-answering systems approximate the human judgments we obtained.

==> backup/introduction_old.tex <==
\section{Introduction}

Text simplification (\ts) aims at rewriting a text such that it is simple to understand compared to the original text for a specific target audience, while preserving the meaning of the original content. A complex text can be simplified by replacing complex or specialized terms with simpler synonyms, restructuring text into short sentences with simple words, deleting redundant or peripheral information, and adding explanations or definitions of complex terminologies \cite{xu2015problems, srikanth-li-2021-elaborative}. The nature and the degree of simplification required are directly dependent upon the target audience and their language proficiency \cite{crossley2014s}. Due to the potential of \ts systems to make texts more accessible to people with various reading or cognitive disabilities, automatically generating a simplified text has been an active area of research in \nlp \cite{chandrasekar-etal-1996-motivations, stajner-2021-automatic}. 

While automatic \ts has been primarily framed as a task that rewrites complex text in simple language in the \nlp literature, in practical applications, it is not sufficient to know that the produced text is simpler. Instead, it might be desirable to measure the extent to which the original text's meaning is preserved in the simplified text \cite{stajner-2021-automatic}. Yet, existing evaluation of automatic \ts systems is primarily carried out by rating the accuracy and simplicity of individual output sentences out-of-context on a scale of 1-to-5 without accounting for the correctness of the simplified text in the context.

An alternative evaluation method uses reading comprehension (RC) exercises to assess the usefulness of automatic \ts systems. Following this method, \newcite{angrosh-etal-2014-lexico, laban-etal-2021-keep} asked human readers to answer questions based on either automatically or manually generated simplified text. While this setup more directly aims at measuring if and to what degree simplified texts can help human readers answer questions about a text \textit{efficiently}, they do not directly account for the errors introduced by automatic \ts systems and their impact on users' performance on RC tasks. \citet{angrosh-etal-2014-lexico}, for example, note that all TS systems evaluated tended to omit information through compression, leading to a decrease in comprehension scores for the text generated by these systems. \mc{need to unpack the last sentence so it is clear what you mean to readers.} \sa{Updated.}

Motivated by the above, in this work, we design a human evaluation of the \textbf{correctness} of text simplification systems based on reading comprehension tasks. \sa{Added:} We focus on evaluating the correctness of model-generated texts as ensuring that the information presented to the users is accurate is key to their deployment in the real world. In our proposed framework, we measure the extent to which people can answer questions about key facts about the original text after reading a simplified version. 

Our key contributions are summarized below:
\begin{enumerate}
    \item We introduce a reading comprehension-based evaluation framework to assess the \textit{correctness} of \ts outputs using multiple-choice question answering.
    \item We conduct a thorough human evaluation using the proposed framework to rank 11 \ts systems (two manual and nine automatic) proposed in prior work.
    \item We study how the system used to answer those questions (human vs question-answering models) impacts the evaluation and the ranking of \ts systems.
    \item We assess existing automatic \ts metrics for their ability in capturing the correctness of the simplified text as measured by the performance on the RC exercises. 
\end{enumerate}

Our research demonstrates that supervised systems that utilize pre-training knowledge achieve the highest level of accuracy in RC tasks compared to other automatic controllable \ts systems. However, we have also observed that these systems fail to maintain the original meaning of the text, resulting in approximately 10\% of the questions being labeled as ``unanswerable'' even for the best-performing supervised system. Our meta-evaluation of commonly used TS automatic metrics reveals that SARI can be a reliable metric for assessing system performance at the paragraph level. Additionally, while model-based question-answering can provide an approximation of system rankings based on human evaluation, we caution that the rankings may be influenced by the impact of \ts on the QA task.


==> backup/reading_framework.tex <==
% placing
\begin{figure*}[htb!]
\centering
\begin{subfigure}{0.95\linewidth}
  \centering
\includegraphics[width=\textwidth]{figures/example_rc.png}
\end{subfigure}%
 \caption{Example Question from OneStopQA. We add an additional answer option (E) to capture non-answerable questions when the questions are paired with an automatically generated simplified text.}\label{fig:example_qa}
\end{figure*}


\section{A Reading Comprehension-based Human Evaluation Framework}


Reading comprehension exercises have been frequently used to gauge users understanding of text material developed by educators or language teachers when engaging with original and human-written simplified texts, where simplified texts have been shown to lead to better text comprehension for L2 learners \cite{long1993modifications,tweissi1998effects, oh2001two, crossley2014s, rets2021simplify},\mc{can you unpack what is learned from each of these papers?} \sa{Added findings for a subset of papers in the list} secondary and post-secondary students 
 \cite{heydari2013effectiveness}. For instance, \citet{long1993modifications} conduct a reading comprehension-based study with 483 Japanese students with varying English language proficiency levels and found that participants who had access to linguistically simplified or elaborated texts scored higher on the RC tasks than the participants who were provided with the original unmodified content. Similarly, \citet{crossley2014s} showed a linear effect of text complexity on comprehension even when accounting for individual language and reading proficiency as well as their background knowledge. Finally, \citet{rets2021simplify}'s study with 37 adult English L2 users showed better comprehension and faster recall for participants with low English proficiency levels with simplified texts.
 
 
 A critical assumption in all the studies is that the simplified text accurately preserves the meaning of the original content and that the RC task can be \textit{solved} by both the original and the modified content. However, this assumption is not always valid when the text is automatically simplified using a model. Automatic text generation models are prone to errors, even at the sentence level, when generating simplified text \cite{devaraj-etal-2022-evaluating}. It is important to note that users' reading comprehension can also be influenced by other factors, such as their background knowledge \cite{young1999linguistic} or familiarity with the topic \cite{rets2021simplify}.\mc{So how does this impact the design of the evaluation?} \sa{We do not directly control for it in our evaluation.} However, errors in the text itself, resulting from incorrect representation of information, can have a notable effect on users' ability to comprehend and interpret the text during reading comprehension tasks.

Hence, in this work, we introduce a human evaluation framework that utilizes reading comprehension exercises to assess the \textit{correctness} of automatically generated text simplification outputs in the context of paragraphs. Our approach involves using multiple-choice questions to evaluate the correctness of the simplified texts, distinguishing it from previous research \cite{laban-etal-2021-keep, angrosh-etal-2014-lexico} that relied on reading comprehension-based human evaluation to measure the \textit{usability} or \textit{efficiency} of text simplification systems without considering the meaning errors introduced by these systems. \mc{You need to explain that contrast better in Section 2, so that here you can just reference the contrast briefly} Our primary focus is on evaluating the \textit{correctness} of simplified texts by employing a question-answering reading comprehension task.

\mc{I think it might be helpful here to have a paragraph on desiderata for the eval task, and then to be concrete and say that here we use OneStopQA (drawing and expanding from what is in the experimental setup; you can leave in the setup section the details on which passages were selected), and show the example.} \sa{Updated}

\paragraph{Desiderata} In order to disentangle the impact of text simplification and the errors introduced in the outputs on the reading comprehension task, we note a few desiderata for the RC task:
\begin{itemize}
    \item The choice of questions and the answer options should enable measuring users' understanding of the content. 
    \item The answer options should potentially include a key containing the correct answer and 3 distractor options that are plausible but incorrect \cite{gierl2017developing}.
    \item  As \ts systems are prone to deleting content from the text which could make reading comprehension questions \textit{unanswerable}, the QA task should ideally be able to capture the failure modes of automatic systems which the participants can select if they cannot answer the question based on the input text provided.
\end{itemize}

We use OneStopQA \cite{berzak-etal-2020-starc} for our evaluation as it matches all the above criteria. Please refer to Section~\ref{subsec:data} for more details.

\paragraph{Design} Given $M$ passages generated from a system $S \in  \{O, H, ATS_1, ... ATS_k\}$, where O is the original unmodified text, H is a human-written simplified rewrite, and ($ATS_1, ATS_2, ... ATS_k$) are simplified texts generated by 
$k$ automatic \ts simplification systems. Each passage $P$ is accompanied by a set of $Q$ questions with 5 multiple-choice answers, $\{q, a_1^5\}_{1}^q$, which includes a correct answer, 3 distractors that reflect the degree of comprehension and a fifth ``unanswerable'' (NA) option that marks the support for the question or the answer options (``The questions or the answer options are not supported by the passage.''). 

\paragraph{Measures} We measure the correctness (C) of the system $S$, $C_S$ using the number of questions answered correctly for that system by human participants. Formally, \mc{Notation is inconsistent (e.g. $C$ vs $C_S$), also yu need to explain intuitively what each metric computes in addition to showing the formulas, and it would be worth defining metrics that chnage in a way that is consistent (eg measure answerability rather than unanswerability, so that both answerability and correctness are higher when the system is better)} \sa{Updated notation and measures need to update the results in section 5.3 accrdingly and also add what they capture.}

\begin{equation} \label{eq:rc_score}
   C_S = \frac{1}{M \times Q} \sum_{m=1}^M \sum_{q=1}^Q 1[ Selected == Correct]
\end{equation}

where Selected is the answer given the passage $P_S$ (either marked by humans or automatic QA systems). We rank the automatic \ts systems based on the ranking induced by $C_S$. 

We also compute answerability for a system $S$, $A_S$ using:

\begin{equation} \label{eq:na_score}
   A_S = 1 - \frac{1}{M \times Q} \sum_{m=1}^M \sum_{q=1}^Q 1[ Selected == NA]
\end{equation}

Intuitively, the questions that are marked ``unanswerable'' (fifth option) directly measure support for the question or the answer option in the passage text (Section~\ref{sec:answerability}) and hence can capture deletion errors, a major error type in \ts outputs \cite{devaraj-etal-2022-evaluating}.  

==> backup/related_work.tex <==
\section{What is missing from current \ts evaluation?}

Several recent works have discussed the limitations of existing automatic and human evaluation techniques in assessing \ts systems. Where automatic metrics fail to capture meaningful differences between simplified texts as suggested by the low correlation of the commonly used TS metrics like BLEU \cite{sulem-etal-2018-bleu}, SARI \cite{alva-manchego-etal-2021-un, maddela2022lens} or the Flesch-Kincaid Grade Level \cite{tanprasert-kauchak-2021-flesch} with human judgments, \mc{Worth unpacking the findings here a bit as motivation rather than do a giant citation dump.} \sa{updated} the progress in developing automatic \ts systems is also impeded by a lack of a standardized human evaluation framework that can measure the \textbf{correctness} (to what extent is the meaning of the original text preserved in the simplified text?) of these systems for target users \cite{stajner-2021-automatic, grabar-saggion-2022-evaluation}.  

Simplified texts that are potentially \textit{unfaithful} or \textit{inaccurate} can cause more harm to end-users, especially in high-risk scenarios (e.g. medical or legal domain) than providing no such access. \citet{devaraj-etal-2022-evaluating} show that factual errors often appear in both human and automatically generated simplified texts (at the sentence level) and propose an error taxonomy to account for both the nature and severity of errors. \citet{maddela2022lens} introduce \textsc{RANK \& RATE}, a human evaluation framework that rates simplifications from several models by leveraging automatically annotated edit operations that are first verified by the annotators and then used to rate the output text on a scale of 0-100 jointly for meaning preservation, simplicity, and fluency. While both approaches intrinsically evaluate the correctness of the model-generated simplified texts, their impact on the reading comprehension of the end users remains unknown. 
\mc{I think the point you are making implicitly here is that correctness has only been evaluated intrinsically via manual annotation, but its impact on reading comprehension is unknown. You need to make that point explicitly.} \sa{Updated the last line to reflect it.}

\citet{angrosh-etal-2014-lexico} were the first to conduct a reading comprehension-based evaluation of \textit{automatically} generated simplified texts generated by multiple \ts models with non-native readers of English. They conduct a multiple-choice reading comprehension test using five news summaries chosen from the Breaking News English website, originally at reading level 6 (hard) and simplified manually or via automatic \ts systems. Their study found no significant differences between the comprehension accuracy of different user groups.
However, they note that the drop in comprehension scores for some of these systems could be accounted to the content removal which can make some questions unanswerable. Hence, it is not clear whether the differences are non-significant due to user understanding, errors introduced by TS systems, or the effectiveness of simplifications. Furthermore, the evaluation was conducted on the simplified outputs generated via non-neural TS models and it is unclear to what extent their findings hold with the newer generation of neural generation systems. \mc{Also this is an older study and it is not clear to what degree their findings hold with the newer generation of neural generation systems.} \sa{Added.}

\mc{Need to use this section to motivate your study much more strongly here. For instance, you should also discuss the Laban et al. paper and any other human studies of TS.} \sa{Added the Laban et al. paper. I discuss some user studies with human simplified texts at the start of the next section }

\citet{laban-etal-2021-keep} also conduct a reading comprehension study to evaluate the usefulness of automatic TS outputs with automatically generated reading comprehension questions that can be answered by original text and human-written references. They found that simplified texts help participants complete the RC task faster than reading original texts. However, their small-scale study only included 3 automatic TS models and 4 documents and allowed users to resubmit based on feedback on questions that were incorrectly answered. They also found that shorter passages generated by automatic TS systems lead to a speed-up regardless of simplicity. We note a few limitations of their study: a) the generated questions were mostly factoid and hence only tested a limited understanding of the text b) they did not account for TS errors which could potentially make the RC questions unanswerable and c) it is unclear how resubmissions impact users understanding. We show that these limitations could potentially impact evaluation as while their results show a significant speedup with KIS simplifications, we show that the outputs generated are unfaithful. 

\textsc{TS} is largely audience-centric \---\ what makes a text simple directly depends upon the target audience. Ideally, the question ``Is the text simple to understand?'' or ``Is the simplified text more readable than the original text?'' when asked to crowdsourced workers who might or might not be the target audience for the simplified texts might not provide a useful signal about the impact of the generated simplified text in \textit{facilitating} the target users' reading comprehension.  As current \ts systems are not designed with a specific target audience in mind and only aim at generating \textbf{a} generic simplified output, in this work, we focus on evaluating the correctness of the generated simplified texts using our proposed framework and leave the exploration of the nature and degree of simplification generated by automatic \ts systems and its impact on target users' reading comprehension to future work.\mc{Not sure whether including this paragraph makes sense since it is not addressed in this paper.} \sa{I am mostly providing reasoning as to why we do not conduct usability evaluation as there is usually no specific target audience for most TS systems, hence answering what is unaddressed and why. We could remove it if it does not make sense.}


% \sa{Discuss \cite{zhou-etal-2022-deconstructing, temnikova-maneva-2013-c }}



